Regularity Conditions for Iterated Shuffle on Commutative Regular Languages

We identify a subclass of the regular commutative languages that is closed under the iterated shuffle, or shuffle closure. In particular, it is regularity-preserving on this subclass. This subclass contains the commutative group languages and, for every alphabet $\Sigma$, the class $\textbf{Com}^+(\Sigma^*)$ given by the ordered variety $\textbf{Com}^+$. Then, we state a simple characterization when the iterated shuffle on finite commutative languages gives a regular language again and state partial results for aperiodic commutative languages. We also show that the aperiodic, or star-free, commutative languages and the commutative group languages are closed under projection.

==> projection.tex <==

Here, we show that for commutative regular languages recognized by 
a commutative automaton with $n$ states, the projection
onto any subalphabet $\Gamma \subseteq \Sigma$
is recognizable by an automaton with $n$ states.
By choosing $\Gamma = \Sigma$, this bound is sharp, even for unary languages, i.e.,
languages with $|\Sigma| = 1$.
An automaton $\mathscr A = (\Sigma, Q, \delta, q_0, F)$
is called \emph{commutative}~\cite{BrzozowskiS73}, if, for any $a,b \in \Sigma$
and state $q \in Q$, we have $\delta(q, ab) = \delta(q, ba)$.


\begin{lemmarep}
\label{lem:com_lang_com_aut}
 Let $L \subseteq \Sigma^*$ be commutative and recognized
 by an automaton with $n$ states.
 Then, there exists a commutative automaton
 with at most $n$ states recognizing $L$.
\end{lemmarep}
\begin{proof}
 Let $\mathscr A = (\Sigma, Q, \delta, q_0, F)$
 be an initially-connected\footnote{An automaton
 $\mathscr A = (\Sigma, Q, \delta, q_0, F)$
 is called \emph{initially-connected}, if for any $q \in Q$,
 there exists $u \in \Sigma^*$ such that $\delta(q_0, u) = q$.
 It is clear that we can omit all states for which no word exists
 that drives the start state to that state. Hence, we can always
 assume an automaton for a given language is initially-connected.}
 finite automaton
 with $|Q| = n$ and $L = L(\mathscr A)$.
 Suppose $\mathscr A$ is not commutative.
 Then, there exists a state $q$ and letters $a,b \in \Sigma$
 such that $\delta(q, ab) \ne \delta(q, ba)$.
 Let $u \in \Sigma^*$ be
 such that $\delta(q_0, u) = q$.
 As $L$ is commutative, for any $v \in \Sigma^*$
 we have
 \begin{equation}\label{eqn:non-comm} 
  \delta(q_0, uabv) \in F \Leftrightarrow \delta(q_0, ubav) \in F.
 \end{equation}
 We use a quotient automaton construction
 described in~\cite{DBLP:books/daglib/0088160}
 to reduce the number of states.
 The procedure in~\cite{DBLP:books/daglib/0088160} 
 only works for complete automata. It could be easily adapted
 to directly work with incomplete input automata,
 but the more easy way is to, if necessary, add a
 sink state to $\mathscr A$ to transform it to a complete
 automaton and then work with this new automaton.
 For simplicity, we simple assume $\mathscr A$
 is complete with at most $n + 1$ states.
 Then, the relation on the states is defined by, for $s,t  \in Q$,
 \[ 
  s \sim t \Leftrightarrow \forall u \in \Sigma^* : \delta(s, u) \in F \Leftrightarrow \delta(t, u) \in F.
 \]
 We see that, for the state $q \in Q$
 above, $\delta(q, ab) \sim \delta(q, ba)$.
 Hence, in the quotient construction, both states
 are put into a single equivalence relation.
 So, the quotient automaton has at most $n$
 states and is complete.
 If the resulting automaton is still not commutative\footnote{Actually, it could be shown that the result must be commutative. In fact, it is the, up to isomorphism, unique minimal automaton.},
 we can repeat the above procedure, were, this time,
 we do not have to add a sink state, as it is already complete.
 So, ultimately, we arrive at a commutative automaton
 with at most $n$ states.~\qed
%  % oder wie in kozen quotient-aut
%  Let $r \notin Q$ be a new state and construct the automaton
%  $\mathcal A' = (\Sigma, Q', \delta', q_0', F')$
%  with, for $s \in Q', x \in \Sigma$,
%  \begin{align*}
%      Q'            & = (Q \setminus \{\delta(q,ab),\delta(q,ba)\}) \cup \{r\} \\
%      \delta'(s, x) & = \left\{ \begin{array}{ll}
%       \delta(s,x)   & \mbox{if } \delta(s,x) \mbox{ is defined and } \{s,\delta(s,x)\} \cap \{\delta(q,ab),\delta(q,ba)\} = \emptyset; \\
%       r             & \mbox{if } \delta(s,x) \in \{\delta(q,ba),\delta(q,ba)\}; \\
%       \delta(s,abx) & \mbox{if } s = r; % todo hier auch definiert hinzufügen.
%      \end{array} \right. \\
%      q_0' & = \left\{
%      \begin{array}{ll}
%       q_0 & \mbox{if } q_0 \notin \{\delta(q,ab),\delta(q,ba)\}; \\
%       r   & \mbox{otherwise};
%      \end{array}\right. \\
%      F' & = \left\{ 
%      \begin{array}{ll}
%       F                      & \mbox{if } F \cap \{\delta(q,ab),\delta(q,ba)\} = \emptyset; \\
%       (F \cap Q') \cup \{r\} & \mbox{otherwise.} 
%      \end{array}
%      \right.
%  \end{align*}
 
%  %
%  % statt neuene zustand r, 
%  % alles was auf delta(q, ba) geht, auf delta(q,ab) umleiten.
 
%  \begin{claiminproof}
%   We have $L(\mathcal A') = L$.
%  \end{claiminproof}
%  \begin{claimproof}
%   First, suppose $\delta'(q_0', u) \in F'$.
  
%   % induktion, wie oft r benutzt in pfad?
%   % ia r = 0 und r = 1, rest einfach
%   %
%   % oder direkt induktion, länge eingabe, wie in kozen
  
%   Conversely, suppose $\delta(q_0, u) \in F'$.
  
  
%   % alternativ, zeigen dass nerode äquivalent -> verschmelzen, aber u.U noch fangzustand dazu, aber hebt sich ja
%   % auf, vielleicht ienfachestes argument

%  \end{claimproof}
 
%  If $\mathcal A'$ is not commutative, we can repeat the above process
%  until we find a commutative automaton, which by construction has 
%  fewer states than $\mathcal A$.~\qed
\end{proof}

Now, our main theorem of this subsection.

\begin{theorem}
 Let $\Gamma \subseteq \Sigma$.
 Suppose $L \subseteq \Sigma^*$ % commutative definiren, und minimal stets commutative
 is recognized by a (possibly incomplete) automaton 
 with $n$ states.
 Then, $\pi_{\Gamma}(L)$
 is recognizable by a commutative automaton with at most $n$
 states.
\end{theorem}
\begin{proof}
 By Lemma~\ref{lem:com_lang_com_aut}, there exists
 a commutative automaton $\mathscr A = (\Sigma, Q, \delta, q_0, F)$
 with $|Q| \le n$ recognizing $L$.
  
 Set $\mathscr B = (\Gamma, S, \delta, q_0, E)$ with\footnote{Note that
 we use the same transition function as in $\mathscr A$, but only
 for inputs from $\Gamma$.} %todo \delta_{\Gamma} einführen! und sagen, im folgenden auch mit gamma
 \begin{align*}
    % \mu(q, x) & = \left\{
    %   \begin{array}{ll} % ist eigentlich gleicher übergang, nur eingeschränkt!
    %     \delta(q, x)     & \mbox{if } \delta(q,x) \mbox{ is defined;} \\ 
    %     \mbox{undefined} & \mbox{if } \delta(q,x) \mbox{ is undefined,} 
    %   \end{array}
    % \right. \\
     S & = \{ \delta(q_0, u) \mid \delta(q_0, u) \mbox{ is defined and } u \in \Gamma^* \}; \\ 
     E & = \{ \delta(q_0, \pi_{\Gamma}(u)) \mid u \in L \}. % note, hier immer definiert, zeigen!
     % oder als fussnote und hinschreiben hinten, dass definiet sein muss
 \end{align*}
 
 \begin{claiminproof}
  We have $\pi_{\Gamma}(L) = L(\mathscr B)$.
 \end{claiminproof}
 \begin{claimproof}
  First, suppose $u \in L(\mathscr B)$.
  Then, $\delta(q_0, u) = \delta(q_0, \pi_{\Gamma}(v))$
  for some $v \in L$.
  As $L$ is commutative, by reordering the letters, 
  there exists a unique $x \in (\Sigma \setminus \Gamma)^*$
  such that $\pi_{\Gamma}(v)x \in \perm(v) \cap L$.
  As \[ \delta(q_0, \pi_{\Gamma}(v)) = \delta(q_0, u), \]
  we find $\delta(q_0, \pi_{\Gamma}(v)x) =  \delta(q_0, ux)$
  and, as $\mathscr A$ is commutative and $\pi_{\Gamma}(v)x \in \perm(v)$,
  we have $\delta(q_0, ux) = \delta(q_0, \pi_{\Gamma}(v)x) = \delta(q_0, v) \in F$.
  Hence $ux \in L$.  
  Set $w = ux$. Then, $u = \pi_{\Gamma}(w)$ and $w \in L$, i.e., $u \in \pi_{\Gamma}(L)$.
  
  
  
  Conversely, suppose $u \in \pi_{\Gamma}(L)$.
  Then, there exists $v \in L$
  such that $u = \pi_{\Gamma}(v)$.
  By commutativity of $\mathscr A$,
  we have $\delta(q_0, \pi_{\Gamma}(v)x) = \delta(q_0, v)$
  for a unique $x \in (\Sigma \setminus \Gamma)^*$
  with $\pi_{\Gamma}(v)x \in \perm(v)$.
  Hence, $\delta(q_0, \pi_{\Gamma}(v))$
  is defined and we find $\delta(q_0, \pi_{\Gamma}(v)) \in E$,
  i.e., $u = \pi_{\Gamma}(v) \in L(\mathscr B)$.
 \end{claimproof}
 As $\mathscr A$ is commutative, also $\mathscr B$
 is commutative and $S \subseteq Q$, which gives the claim.~\qed
\end{proof}

% Todo, noch mit index und period schranke. % aberf olgt doch, da obere schranke das produkt für n
% aber so wie in nis schreiben.



